Robust Retrieval Augmented Generation for Zero-shot Slot Filling

Automatically inducing high quality knowledge graphs from a given collection of documents still remains a challenging problem in AI. One way to make headway for this problem is through advancements in a related task known as slot filling. In this task, given an entity query in form of [Entity, Slot, ?], a system is asked to fill the slot by generating or extracting the missing value exploiting evidence extracted from relevant passage(s) in the given document collection. The recent works in the field try to solve this task in an end-to-end fashion using retrieval-based language models. In this paper, we present a novel approach to zero-shot slot filling that extends dense passage retrieval with hard negatives and robust training procedures for retrieval augmented generation models. Our model reports large improvements on both T-REx and zsRE slot filling datasets, improving both passage retrieval and slot value generation, and ranking at the top-1 position in the KILT leaderboard. Moreover, we demonstrate the robustness of our system showing its domain adaptation capability on a new variant of the TACRED dataset for slot filling, through a combination of zero/few-shot learning. We release the source code and pre-trained models.

==> dns2.tex <==
%In addition, we also technique to generate negative examples for DPR, called Dense Negative Sampling. DNS gathers hard negatives for DPR training, with one difference: rather than locating the hard negative passages by BM25, it find relevant passages by ANN search over the learned index.  The intuition is ... \todo{Michael describe why we do that}
%We train for an additional two epochs using these hard negatives. As Figure \ref{fig.arch} shows, the DPR question encoder is trained both by DPR and later by RAG. 

\subsection{Dense Negative Sampling for DPR}


The negative sampling procedure can have a large impact on the performance of a dense retrieval system \cite{samplingMatters}. We start observing that RAG training is using the weak supervision of the passage's impact in producing the correct answer, rather than the ground truth provenance of DPR training, which is likely a disadvantage. In addition, the other key difference between DPR and RAG training is that RAG uses negatives drawn from the trained index rather than from BM25. 

Motivated by this observation, we further explored additional ways to train DPR in combination with RAG.

We index the passages using the KILT trained DPR models. Then we gather hard negatives for DPR training, with one difference: rather than locating the hard negative passages by BM25, we find the passage by ANN search over the learned index: Dense Negative Sampling.  We applied this step of constructing a temporary passage index to gather negatives for further training only once, although it could also be done for each epoch. We train for an additional two epochs using these hard negatives. Once the DPR training completes, the temporary passage index is discarded and the passages are re-indexed with the final context encoder model from DPR. We call this technique Dense Negative Sampling (DNS).

Table \ref{tbl.retrieval} shows the performance of the different approaches to retrieval. DPR$_{NQ}$ is the DPR model pre-trained on Natural Questions. DPR$_{BM25}$ further trains DPR$_{NQ}$ on the KILT data with BM25 hard negatives. Rows with +RAG further train the question encoder through RAG.  The row DPR$_{DNS}$ (\textbf{D}ense \textbf{N}egative \textbf{S}ampling) shows the performance of retrieval immediately after DNS training. Surprisingly, this results in lower performance for T-REx relative to DPR$_{BM25}$. However, further training the DNS model with RAG results in our best performance for both T-REx and zsRE.

\begin{table}[t]
\small
\begin{center}
\begingroup
\renewcommand{\arraystretch}{1.2} 
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|cc|cc}
 & \multicolumn{2}{c|}{\textbf{T-REx}} & \multicolumn{2}{c}{\textbf{zsRE}}\\\hline
& \textbf{R-Prec}  & \textbf{R@5} & \textbf{R-Prec}  & \textbf{R@5} \\
\hline
DPR$_{NQ}$ & 19.50 & 29.80 & 45.49 & 60.77 \\
DPR$_{NQ}$+RAG & 53.04 & 65.54 & 68.13 & 79.19 \\
DPR$_{BM25}$ & 49.02 & 63.34 & 94.55 & 98.17 \\
DPR$_{BM25}$+RAG & 65.02 & 75.52 & 96.89 & 98.01 \\
DPR$_{DNS}$ & \textit{42.62} & \textit{55.09} & 97.53 &	99.30 \\
DPR$_{DNS}$+RAG & \best{74.34} & \best{82.89} & \best{98.60} & \best{99.70}
\end{tabular}
}
\endgroup
\end{center}
\caption{\label{tbl.retrieval}Retrieval performance of DPR and RAG on Dev sets}
\end{table}

After training with DNS the FAISS indexing with scalar quantization becomes prohibitively slow.  We therefore remove all quantization and use four shards (the index is split into four, with the results of each query merged) for our experiments with DNS enabled KGI.


==> dns3.tex <==
As Figure \ref{fig.arch} shows, the DPR question encoder is trained both by DPR and later by RAG. To examine the influence of this additional training from RAG on the retrieval performance, we compare retrieval metrics before and after RAG fine-tuning.  Table \ref{tbl.retrieval} shows the large gains from training with RAG after DPR. 
Note that RAG training is using the weak supervision of the passage's impact in producing the correct answer, rather than the ground truth provenance of DPR training. Since this is likely a disadvantage, we explore the other key difference with DPR and RAG training: RAG uses negatives drawn from the trained index rather than from BM25.

\subsection{Dense Negative Sampling}


\begin{table}[thb]
\small
\begin{center}
\begingroup
\renewcommand{\arraystretch}{1.2} 
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|cc|cc}
 & \multicolumn{2}{c|}{\textbf{T-REx}} & \multicolumn{2}{c}{\textbf{zsRE}}\\\hline
& \textbf{R-Prec}  & \textbf{R@5} & \textbf{R-Prec}  & \textbf{R@5} \\
\hline
DPR$_{NQ}$ & 19.50 & 29.80 & 45.49 & 60.77 \\
DPR$_{NQ}$+RAG & 53.04 & 65.54 & 68.13 & 79.19 \\
DPR$_{BM25}$ & 49.02 & 63.34 & 94.55 & 98.17 \\
DPR$_{BM25}$+RAG & 65.02 & 75.52 & 96.89 & 98.01 \\
DPR$_{DNS}$ & \textit{42.62} & \textit{55.09} & 97.53 &	99.30 \\
DPR$_{DNS}$+RAG & \best{74.34} & \best{82.89} & \best{98.60} & \best{99.70}
\end{tabular}
}
\endgroup
\end{center}
\caption{\label{tbl.retrieval}Analysis of retrieval by DPR and RAG on Dev}
\end{table}

In this subsection we propose an improvement to the DPR training procedure that we call Dense Negative Sampling (DNS). Using the KILT trained DPR models, we index the passages. Then we gather hard negatives for DPR training, with one difference: rather than locating the hard negative passages by BM25, we find the passage by ANN search over the learned dense vector index.  We train for an additional two epochs using these hard negatives. 
%The intuition is that following this procedure we further increase the ability of DPR to find relevant passages for the short slot filling queries beyond keyword matching.
%consisting on only the subject entity and the required relation.  

After training with DNS the FAISS indexing with scalar quantization becomes prohibitively slow.  We therefore remove all quantization and use four shards (the index is split into four, with the results of each query merged) for our experiments with DNS enabled KGI.


Table \ref{tbl.retrieval} shows an analysis of the performance of the different approaches to retrieval. DPR$_{NQ}$ is the DPR model pre-trained on Natural Questions. DPR$_{BM25}$ further trains DPR$_{NQ}$ on the KILT data with BM25 hard negatives. Rows with +RAG further train the question encoder through RAG.  The row DPR$_{DNS}$ (\textbf{D}ense \textbf{N}egative \textbf{S}ampling) shows the performance of retrieval immediately after DNS training. Surprisingly, this results in lower performance for T-REx relative to DPR$_{BM25}$. However, further training the DNS model with RAG results in our best performance for both T-REx and zsRE.
Since RAG does not update the context encoder, DNS training is the only training for the context encoder when negatives are drawn from the dense vector index.



==> kilt_analysis.tex <==
To explore the effect of retrieval performance on downstream performance we consider two variants of our systems: one using random passages from the index and another using passages from the ground truth provenance. Table \ref{tbl.goldRandom} compares three systems, differing only in the retrieval used for training. By supplying these systems with the gold standard passages, we can see both the improvement possible through better retrieval, but also the value of good retrieval during training. The best system, $KGI_1$ is the most effective at generating slot fillers from relevant explicit knowledge because it was trained on more cases of justifying explicit knowledge. However, given random passages it is the worst. It has sacrificed some implicit knowledge for better capabilities in using explicit knowledge.

\begin{table}[t]
\small
\begin{center}
\begingroup
\renewcommand{\arraystretch}{1.2} 
\begin{tabular}{r|ccc}
Passages & $RAG_{NQ}$ & $KGI_0$ & $KGI_1$\\
\hline
Retrieved & 70.58 & 76.58 & 84.04 \\
\hline
Gold &      88.66 & 89.46 & \best{90.20} \\
Random &    38.84 & \best{39.26} & \textit{36.64}
\end{tabular}
\endgroup
\end{center}
\caption{\label{tbl.goldRandom}T-REx Accuracy with Random and Gold Retrieval}
\end{table}

%T-REx
% NQ             70.58%		74.74%
% NQ (gold)      88.66%		91.27%
% $KGI_0$        76.58%		80.27%
% $KGI_0$ (gold) 89.46%		91.80%
% $KGI_1$        84.04%		86.89%
% $KGI_1$ (gold) 90.20%		92.44%

% $BART_{LARGE}$  43.84%		48.25%
% NQ (random)      38.84%		45.47%
% $KGI_0$ (random) 39.26%		45.54%
% $KGI_1$ (random) 36.64%		43.32%

%zsRE
% BART_LARGE 9.14% acc on test
% NQ             46.03%		55.75%
% NQ (gold)      76.48%		83.72%
% $KGI_0$        69.47%		77.24%
% $KGI_0$ (gold) 77.18%		84.51%
% $KGI_1$        71.32%		78.85%
% $KGI_1$ (gold) 77.58%		84.45%

Relative to the best implicit-knowledge system for KILT slot filling, BART$_{LARGE}$, $KGI_1$ makes large gains - over 40 points in accuracy on T-REx Dev. To understand the impact of the explicit knowledge used by $KGI$ we examine the improvement over BART$_{LARGE}$. We consider two main hypotheses: the value of explicit knowledge depends on the relation, and the value of explicit knowledge depends on the corpus frequency of the entities related.

To understand the impact of relation-type on the effectiveness of explicit knowledge, we consider the most frequent twenty relations in the T-REx Dev set; each occurs at least 40 times. The relations with the lowest relative performance gain are taxonomy and partonomy relations: \relation{taxon-rank}, \relation{subclass-of}, \relation{instance-of}, \relation{part-of} and \relation{parent-taxon} as well as \relation{languages-spoken,-written-or-signed} and \relation{sport}. Inspecting the \relation{languages-spoken,-written-or-signed} we find that surface level information (i.e. French name vs. Russian name) is often sufficient for the correct prediction.  For \relation{sport} we see cases where the answer is in the head entity (i.e. `batminton' in `2000 European Badminton Championships').

In contrast, the relations that gain the most from explicit knowledge are: \relation{performer}, \relation{member-of-sports-team}, \relation{author}, \relation{place-of-birth}, \relation{country-of-origin}, \relation{cast-member}, \relation{director}. These relations are not central to the meaning of the head entity, like the taxonomy and partonomy relations, and are not typically predictable from surface-level features. 

Regarding our second hypothesis, we might expect that more frequent entities have better representations in the parameters of a pre-trained language model, and that therefore implicit knowledge will show a strong dependence on the corpus frequency of the head or tail entity. 

To test it, we used simple dictionary matching to find a count of all entities, both head and tail in the T-REx development set. We group the Dev instances according to the decile of the head or tail entity frequency. We compute a macro-accuracy, weighting all relations equally rather than by their frequency.  Figure \ref{fig.entFreq} shows the macro-accuracy of BART$_{LARGE}$ and $KGI_1$ for each decile of head and tail entity frequency. Although there is a general trend of higher accuracy for more frequent tail entities and lower accuracy for more frequent head entities, \textit{there is no pattern to the gain of explicit knowledge over implicit knowledge from entity frequency}.  
%Considering the minimum frequency for the head or tail entity gives a similar picture. 
This falsifies our second hypothesis and suggests implicit knowledge is distinct in kind from explicit knowledge, rather than merely under-trained for low frequency entities.


\begin{figure}[thb]
   \centering
   \includegraphics[width=0.95\linewidth]{figures/KGI_vs_BART_entity_freq.pdf}
   \caption{Performance as a function of entity frequency}
   \label{fig.entFreq}
\end{figure}


==> kilt_experiments_old.tex <==
Table \ref{tbl.datasets} gives statistics on the two zero-shot slot filling datasets in KILT. While the T-REx dataset is larger by far in the number of instances, the training sets have a similar number of distinct relations. We use only 500k training instances of T-REx in our experiments to increase the speed of experimentation.

\begin{table}
\begin{center}
\begingroup
\renewcommand{\arraystretch}{1.2} 
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|ccc|ccc}
 & \multicolumn{3}{c|}{\textbf{Instances}} & \multicolumn{3}{c}{\textbf{Relations}}\\ \hline
\textbf{Dataset} & \textbf{Train}  & \textbf{Dev} & \textbf{Test} & \textbf{Train}  & \textbf{Dev} & \textbf{Test}\\
\hline
%zsRE  &	147909 & 3724 & 4966 &	84 & 12 & 24 \\
%T-REx &	2284168 & 5000 & 5000 &	106 & 104 & 104
zsRE  &	148K & 3724 & 4966 &	84 & 12 & 24 \\
T-REx &	2284K & 5000 & 5000 &	106 & 104 & 104
\end{tabular}
}
\endgroup
\end{center}
\caption{\label{tbl.datasets}Slot filling datasets in KILT}
\end{table}

Since the transformers for passage encoding and generation can accept a limited sequence length, we segment the documents of the KILT knowledge source (2019/08/01 Wikipedia snapshot) into passages. The ground truth provenance for the slot filling tasks is at the granularity of paragraphs, so we align our passage segmentation on paragraph boundaries when possible.  If two or more paragraphs are short enough to be combined, we combine them into a single passage and if a single paragraph is too long, we truncate it.

% CONSIDER: move to appendix?
%Because the evidence used is at the level of passages but the evaluation is on page level retrieval, we retrieve up to twenty passages so that we typically get at least five documents for the Recall@5 metric.

\subsection{Slot Filling Experiments}

As an initial experiment we tried RAG with its default index of Wikipedia, distributed through Hugging Face. We refer to this as RAG-KKS, or RAG without the KILT Knowledge Source, as reported in Table \ref{tbl.dev}. Since the passages returned are not aligned to the KILT provenance ground truth, we do not report retrieval metrics for this experiment.  

Motivated by the low retrieval performance reported for the RAG baseline by \citet{kilt}, we experimented with replacing the DPR retrieval with simple BM25 (RAG+BM25) over the KILT knowledge source. We provide the raw BM25 scores for the passages to the RAG model, to weight their impact in generation. We also experimented with the Natural Questions trained DPR, with only RAG training on KILT (RAG+DPR$_{NQ}$). To examine the influence of this additional training from RAG on the retrieval performance, we compare retrieval metrics before and after RAG fine-tuning. 

We use the approach explained in Section \ref{sec.approach} to train both the DPR and RAG models. We call the system without DPR trained using hard negative samples from BM-25 index $KGI_0$, an initial knowledge graph induction system.  The successor system, $KGI_1$ incorporates DPR training using hard negatives mined from the index.

The metrics we report include accuracy and F1 on the slot filler, where F1 is based on the recall and precision of the tokens in the answer - allowing for partial credit on slot fillers.  Our systems (except for RAG-KKS) also provide provenance information for the top answer.  R-Precision and Recall@5 measure the quality of this provenance against the KILT ground truth provenance.  Finally, KILT-Accuracy and KILT-F1 are combined metrics that measure the accuracy and F1 of the slot filler \textit{only when the correct provenance is provided}. 
Table \ref{tbl.dev} gives our development set results.

\begin{table}[t]
\begin{center}
\small
\begingroup
\renewcommand{\arraystretch}{1.2} 
\begin{tabular}{r|cccc}
& \textbf{R-Prec}  & \textbf{R@5} & \textbf{Acc.} & \textbf{F1} \\
\hline \multicolumn{5}{c}{\textbf{zsRE}} \\ \hline
RAG-KKS  &	 &  & 38.72 & 46.94\\
% 45.73%		55.18%	58.86%	80.24%
RAG+BM25 &	58.86 & 80.24 & 45.73 & 55.18  \\
% 46.03%		55.75%	68.13%	79.19%
RAG+DPR$_{NQ}$ & 68.13 & 79.19 & 46.03 & 55.75 \\
% 69.47 	77.24%	96.24%	97.53%
$KGI_0$ & 96.24 & 97.53 & 69.58 & 77.24  \\
% 71.32%		78.85%	98.60%	99.70%
$KGI_1$ & \best{98.60} & \best{99.70} & \best{71.32} & \best{78.85} \\	
\hline \multicolumn{5}{c}{\textbf{T-REx}} \\ \hline
RAG-KKS  &	 &  & 63.28 & 67.67   \\
% 69.10%		73.11%	46.40%	67.31%
RAG+BM25 &	46.40 & 67.31 & 69.10 & 73.11  \\
% 73.02%		76.97%	53.04%	65.54%
RAG+DPR$_{NQ}$ & 53.04 & 65.54 & 73.02 & 76.97 \\
% 76.58%	80.27%	61.30%	71.18%
$KGI_0$ & 61.30 & 71.18 & 76.58 & 80.27 \\  
% 84.04%		86.89%	74.34%	82.89%
$KGI_1$ & \best{74.34} & \best{82.89} & \best{84.04} & \best{86.89}
\end{tabular}
\endgroup
\end{center}
\caption{Dev sets performance for different retrieval methods}
\label{tbl.dev}
\end{table}

\begin{table*}[t]
\begin{center}
%\resizebox{0.8\linewidth}{!}{%
\small
\begingroup
\renewcommand{\arraystretch}{1.2} 
\begin{tabular}{r|ccccccc}
 & \textbf{R-Prec}  & \textbf{Recall@5} & \textbf{Accuracy} & \textbf{F1}  & \textbf{KILT-AC} & \textbf{KILT-F1}\\
\hline \multicolumn{7}{c}{\textbf{zsRE}} \\ \hline
$KGI_{1}$ & \best{98.49} & \best{99.23} & \best{72.55} & \best{77.05} & \best{72.31} & \best{76.69} \\
$KGI_{0}$  & 94.18 & 95.19 & 68.97 & 74.47 & 68.32 & 73.45 \\
DensePhrases & 57.43 & 60.47 & 47.42 & 54.75 & 41.34 & 46.79 \\
GENRE & 95.81 & 97.83 & 0.02 & 2.10 & 0.00 & 1.85 \\
Multi-DPR & 80.91 & 93.05 & 57.95 & 63.75 & 50.64 & 55.44 \\
RAG {\small (KILT organizers)} & 53.73 & 59.52 & 44.74 & 49.95 & 36.83 & 39.91 \\
BART$_{LARGE}$ & N/A & N/A & 9.14 & 12.21 & N/A & N/A \\
\hline \multicolumn{7}{c}{\textbf{T-REx}} \\ \hline
$KGI_{1}$  & 74.36  & 83.14 & \best{84.36} & \best{87.24} & \best{69.14} & \best{70.58} \\
$KGI_{0}$  & 59.70 & 70.38 & 77.90 & 81.31 & 55.54 & 56.79 \\
DensePhrases & 37.62 & 40.07 & 53.90 & 61.74 & 27.84 & 32.34 \\
GENRE &	\best{79.42} & \best{85.33} & 0.10 & 7.67 & 0.04 & 6.66 \\
Multi-DPR & 69.46 & 83.88 & 0.00 & 0.00 & 0.00 & 0.00 \\
RAG {\small (KILT organizers)} &	28.68 & 33.04 & 59.20 & 62.96 & 23.12 & 23.94 \\
BART$_{LARGE}$ & N/A & N/A & 45.06 & 49.24 & N/A & N/A
\end{tabular}
\endgroup
\end{center}
\caption{KILT leaderboard top systems performance on slot filling tasks}
\label{tbl.test}
\end{table*}

Table \ref{tbl.test} gives the test set performance of the top systems on the KILT leaderboard.  $KGI_0$ and $KGI_1$ are our systems, while DensePhrases, GENRE, Multi-DPR and RAG for KILT are explained briefly in Section \ref{sec.related}.  $KGI_1$ gains dramatically in slot filling accuracy over the previous best systems, with gains of over 14 percentage points in zsRE and even more in T-REx.  The combined metrics of KILT-AC and KILT-F1 show even larger gains, suggesting that the $KGI_1$ approach is effective at providing justifying evidence when generating the correct answer.  We achieve gains of 21 to 41 percentage points in KILT-AC.
% CONSIDER: maybe these sentences should move to the conclusion

% optional commentary
Relative to Multi-DPR, we see the benefit of weighting passage importance by retrieval score and marginalizing over multiple generations, compared to the strategy of concatenating the top three passages and running a single sequence-to-sequence generation. %Also, fine tuning the query encoder through end-to-end training of tail entity generation produces large gains over DPR alone. 
GENRE is still best in retrieval for T-REx, suggesting that at least for a corpus such as Wikipedia, generating the title of the page can be very effective. A possible explanation for this behaviour is that most relations for a Wikipedia entity are mentioned in its corresponding page.
